Blind Dynamic Resource Allocation in Closed Networks via Mirror Backpressure

We study the problem of maximizing payoff generated over a period of time in a general class of closed queueing networks with a finite, fixed number of supply units which circulate in the system. Demand arrives stochastically, and serving a demand unit (customer) causes a supply unit to relocate from the ``origin'' to the ``destination'' of the customer. The key challenge is to manage the distribution of supply in the network. We consider general controls including customer entry control, pricing, and assignment. Motivating applications include shared transportation platforms and scrip systems. Inspired by the mirror descent algorithm for optimization and the backpressure policy for network control, we introduce a rich family of \emph{Mirror Backpressure} (MBP) control policies. The MBP policies are simple and practical, and crucially do not need any statistical knowledge of the demand (customer) arrival rates (these rates are permitted to vary in time). Under mild conditions, we propose MBP policies that are provably near optimal. Specifically, our policies lose at most $O(\frac{K}{T}+\frac{1}{K} + \sqrt{\eta K})$ payoff per customer relative to the optimal policy that knows the demand arrival rates, where $K$ is the number of supply units, $T$ is the total number of customers over the time horizon, and $\eta$ is the demand process' average rate of change per customer arrival. An adaptation of MBP is found to perform well in numerical experiments based on data from ride-hailing.

==> 1-intro-backup.tex <==
\section{Introduction}\label{sec:intro}
The control of complex systems with circulating resources such as shared transportation platforms and scrip systems has been heavily studied in recent years.
%
The hallmark of such systems is that serving a demand unit causes a (reusable) supply unit to be relocated.
Closed queueing networks (i.e., networks where a fixed number of supply units circulate in the system) provide a powerful abstraction for these applications \citetext{\citealp*{banerjee2016pricing}, \citealp{braverman2016empty}}. The key challenge is \emph{managing the distribution of supply} in the network.
%
A widely adopted approach for this problem is to solve the deterministic optimization problem that arises in the continuum limit (often called \emph{the static planning problem}), and show that the resulting control policy is near-optimal in a certain asymptotic regime.
%
However, this approach only works under the restrictive assumption that \emph{(1) the system parameters (demand arrival rates) are precisely known}. Furthermore, previous papers
\citetext{\citealp*{banerjee2016pricing}, \citealp{braverman2016empty}} assume that \emph{(2) the system is in steady state}.
%
As is pointed out by \citet*{banerjee2016pricing}, relaxing either of these assumptions has been of interest.
%

In this paper, we relax \emph{both} assumptions.\footnote{The paper \citet*{banerjee2018SMW} is similarly motivated, but restricts attention to a narrow special case: assignment control in networks satisfying a strong \emph{complete resource pooling} (CRP) assumption, and conducts a sharp large deviations analysis. In particular, non-idling/greedy policies suffice to achieve asymptotic optimality under CRP. In contrast, the present work is general: e.g., the JEA setting we solve in Section~\ref{sec:extension} generalizes the model of that paper by dropping the CRP assumption, necessitating a completely different non-greedy approach to control; already under our illustrative model (Section~\ref{sec:model}) the CRP assumption of \citet*{banerjee2018SMW} is automatically violated and the greedy policy fails to achieve asymptotic optimality.\pqr{Shall we delete this footnote, since no one is asking about it?}}
We propose a family of simple, practical control policies that are \emph{blind} in that they use \emph{no} prior knowledge of demand arrival rates, and prove strong transient and steady state performance guarantees for these policies, for time-varying demand arrival rates.
%that are stationary or vary slowly in time.
In simulations, our policies achieve excellent performance that beats the state-of-the-art policies even in an unequal contest where the latter policies are provided exact demand arrival rates whereas our proposed policies are given \emph{no} prior information about demand arrival rates.

\smallskip
\textbf{Informal description of the model.}
%For ease of exposition, 
Our main setting is one where the control levers include entry control and flexible assignment of resources, with time-varying demand arrival rates.
%is the only available control lever, and demand is stationary.
Later we allow other controls such as dynamic pricing %of relocating resources,
%and 
%(see Section \ref{sec:model} for detailed description of different settings and their corresponding applications).
and show that our machinery and guarantees extend seamlessly.
In our main joint entry-assignment control model, we consider a closed queueing network that consists of $m$ nodes (locations), and a fixed number $K$ of supply units that circulate in the system.
%
Demand units with different types, where each type has an associated pick-up and drop-off neighborhood, arrive stochastically over slotted time with some time-varying arrival rates which are unknown to the controller.
The controller dynamically decides whether to admit each incoming demand unit, and where to pick up and drop off the admitted demand.
%
Each control decision has two effects: it generates a certain \textit{payoff} depending on the type of the demand unit and the pick-up/drop-off location, and it causes a supply unit to \textit{relocate} from the pick-up node to the drop-off node instantaneously, if the pick-up node is non-empty.
The goal of the system is to maximize the collected payoff over a period of time.
%\textcolor{red}{[Greedy policy loses $\Omega(1)$]}

Notably, the greedy policy, which admits a demand unit if a supply unit is available in its pick-up neighborhood, is generically far from optimal: even as $K \rightarrow \infty$, the optimality gap per demand unit of this policy is $\Omega(1)$ even in steady state; see Remark~\ref{rem:CRP-is-violated-and-greedy-is-suboptimal} in Section~\ref{sec:model}. The intuition is that some nodes have no available supply an $\Omega(1)$ fraction of the time in steady state under the greedy policy, and so the policy is forced to drop a significant proportion of the demand which would have been served under the optimal policy.
Furthermore, if demand arrival rates are imperfectly known, any state independent policy \citep*[such as that of][]{banerjee2016pricing} generically suffers a steady state optimality gap per demand unit of $\Omega(1)$; see \citet*[][Proposition~4]{banerjee2018SMW}. %(as $K \rightarrow \infty$).


\smallskip
\textbf{Preview of our main result.}
%We now give a preview of our main performance guarantee.
%Define the optimality gap of a policy to be the fraction of the achievable payoff it loses comparing to the optimal dynamic policy that has access to system parameters and all past information.
%
We propose a large class of simple and practical control policies that are blind (i.e., require \emph{no} estimates of the demand arrival rates), and show that, under a mild connectivity assumption on the network, the policies are near optimal. Specifically, we show that our policies lose payoff (per demand unit) %the optimality gap (per demand unit) relative to polici is bounded above as
%\begin{align*}
at most $
O\left(\frac{K}{T} + \frac{1}{K} + \sqrt{\eta K}\right)$ relative to the optimal policy that knows the demand arrival rates, %\end{align*}
where $K$ is the number of supply units, $T$ is the number of demand units that arrive during the period of interest, and $\eta$ is the average change in demand arrival rates per customer arrival. %(hence $K/T = \Theta(1/T^{\textup{real}})$ where $T^{\textup{real}}$ is physical time.
Our result is \textit{non-asymptotic}, i.e., our performance guarantee holds for finite $K$ and $T$,  and thus covers both transient and steady state performance.
In particular, for stationary demand arrivals, taking $T\to\infty$, we obtain a steady state optimality gap of $O(\frac{1}{K})$, matching that of the state-of-the-art policy of \citet*{banerjee2016pricing}, though that policy requires perfect estimates of demand arrival rates, %\footnote{As shown in \citet*[][Proposition~4]{banerjee2018SMW}, if the estimate of demand arrival rates is imperfect, any state independent policy \citep*[such as that of][]{banerjee2016pricing} will generically suffer a long run (steady state) per period optimality gap of $\Omega(1)$ (as $K \rightarrow \infty$).}
in sharp contrast to our policy which is completely blind. 
Our bound further provides a guarantee on transient performance: the horizon-dependent term $K/T$ in our bound on optimality gap is small if the total number of arrivals $T$ over the horizon is large compared to the number of supply units $K$. 
Our policies retain their good performance if the average change of demand arrival rates over $K$ periods, i.e., the term $\eta K$, is small.
Notably, our bound does not deteriorate as the system size increases in the ``large market regime'' where the number of supply units $K$ increases proportionally to the demand arrival rates (see the discussion after Theorem~\ref{thm:main_regret}):
%	Define $T^{\textup{real}}$ as the physical time for a system with $K$ vehicles.
%	As $K$ increases in the large market regime, the primitive $\bphi$ remains unchanged, while
here the number of arrivals $T = \Theta(K\cdot T^{\textup{real}})$, where $T^{\textup{real}}$ is the time horizon measured in physical time, $\zeta \triangleq \eta K$ is average rate of change of $\bphi$ with respect to physical time, we can rewrite our bound on the optimality gap as
	$
	O\left(\frac{1}{T^{\textup{real}}} +
	\frac{1}{K} + \sqrt{\zeta} \right ) \xrightarrow{K \to \infty} O\left(\frac{1}{T^{\textup{real}}} + \sqrt{\zeta}\right )
	$.
	%where the horizon-dependent term $\frac{M}{T^{\textup{real}}}$ is scale-invariant as $K$ increases.
%As we discuss subsequent to stating our main result, in a ``large market regime'' where $T$ is assumed to scale up linearly with $K$ as per $T = $%\yk{It's a bit dissatisfying that we don't comment on the $K/T$ term.}
%\pqr{Foreshadowing the Remark 2 about $K/T$.}

%Our policies retain their good performance if demand arrival rates vary slowly over time: We show (see Section~\ref{subsec:jea}) that the loss in payoff per customer under MBP is bounded by $O\left(\frac{K}{T} + \frac{1}{K} + \sqrt{\eta K}\right)$, where is $\eta$ is the maximum change in demand arrival rates per customer arrival. In the aforementioned large market regime,  the optimality gap per customer can be expressed as $O\left (\frac{1}{T^{\textup{real}}} + \frac{1}{K} + \sqrt{\zeta} \right )$ where $\zeta \triangleq \eta K$ is rate of change of $\bphi$ with respect to physical time.

We now motivate and introduce our control policies. First, we describe how our problem is one of controlling a closed queueing network. Next, we describe the celebrated backpressure methodology for blind control of queueing networks. We then outline the central challenge in using backpressure in settings like ours. Finally, we introduce our proposed policies which significantly generalize backpressure, and may be broadly useful.
%Our work fits into the broad literature on the control of stochastic processing networks \citep{harrison2000brownian,harrison2003broader}, and our methodology of designing blind control policies and obtaining provable guarantees applies to open queueing networks as well.

\smallskip
\textbf{Analogy with control of a closed queueing network.}
Our problem can be viewed as one of optimal control of a closed queueing network. In the terminology of classic queueing theory, the $\N$ supply units are ``jobs'', and each node has a queue of jobs (supply units).
Each demand type is a ``server'' which receives a ``service token'' each time a demand unit of that type arrives. 
(We emphasize the reversal of the usual mapping: in our setup supply units are ``jobs'' and demand units act as service tokens.) 
The flexible assignment control corresponds to the ``scheduling'' and ``routing'' of jobs.
%Our model also specifies the ``routing'' of jobs: service tokens are labeled with a destination queue to which the served job (supply unit) moves.
Since jobs circulate in the system (they do not arrive or leave), our setup is a \emph{closed} queueing network.\footnote{There are subtle differences between our model and ``classical'' closed queueing networks in the timing of when a job joins the destination queue, and when the ``service'' of a job is initiated. These differences are non-essential, see, e.g., \citet*[Section~8]{banerjee2018SMW}.} (Networks where jobs arrive, go through one or more services, and then leave, are called \emph{open} networks.)  %As a consequence, intuition based on traditional queueing systems does not easily extend to our setup.} %, each supply location is a ``buffer'',
%inter-arrival times of customers with origin $i$ are ``service times'' at server $i$.
%The distribution of customers' destinations given an origin captures ``routing probabilities''.
%``Servers'' are flexible (i.e. can serve multiple queues), and assignment is equivalent to ``scheduling''.



%

%We consider the control problem of shared transportation platforms for ride-hailing such as Uber, Lyft, DiDi and Ola.
%These platforms can be modeled as dynamic two-sided markets where demand units (customers) with different origin-destination pairs arrive stochastically over time.
%The system dynamically decides which customers to serve (or sets prices) and assigns supply units (vehicles) to customers based on the current system state.
%(For example, Didi in China does not use dynamic pricing to manage demand-supply imbalances. Instead it serves customers selectively, e.g., by showing a long wait time to customers in under-supplied locations, causing many such customers to abandon. In contrast, dynamic pricing is the most popular control lever in North America, Europe, etc.) %, in the face of the complication caused by queueing network dynamics.
\smallskip
\textbf{Backpressure.}
Our control approach is inspired by the celebrated backpressure methodology of \citet{tassiulas1992stability} for the control of queueing networks. Backpressure simply uses queue lengths as congestion costs (the shadow prices to the flow constraints; the flow constraint for each queue is that the inflow must be equal to the outflow in the long run), and chooses a control decision at each time which maximizes the myopic payoff inclusive of congestion costs. Concretely, in the special case where entry control is the only leverage, backpressure admits a demand if and only if the payoff of serving the demand plus the origin queue length exceeds the destination queue length.
This simple approach has been used very effectively in a range of %practical and theoretical
settings arising in cloud computing, networking, etc.; see, e.g. \cite{georgiadis2006resource}.
Backpressure is provably near-optimal (in the large market limit) in many settings where payoffs accrue from serving jobs, because it has the property of executing dual stochastic gradient descent (SGD) on the controller's deterministic (continuum limit) optimization problem.
As we discuss next, this property breaks down when the so-called ``no-underflow constraint'' binds, making it very challenging to use backpressure in our setting (indeed, this difficulty appears to be the reason that backpressure has not yet been proposed as a control approach in such settings with circulating resources).

\smallskip
\textbf{Main challenge: no-underflow constraint.}
The control policy must satisfy the \emph{no-underflow constraint}, namely, that each decision to admit a demand unit needs to be backed by an available supply unit at the pick-up node of the demand. This constraint couples together the present and future decisions, and presents a challenge in deploying the backpressure methodology in numerous settings, including ours.

In certain settings this constraint does \emph{not} pose a problem: For example, in the well known ``crossbar switch'' problem in \cite{maguluri2016heavy}, there are no ``payoffs'' apart from the shadow prices (the goal is only to prevent queues from building up), so backpressure only recommends to serve a queue with positive length (after all, backpressure only serves a queue if it is longer than the destination queue) and so the no-underflow constraint does not bind.
In several works that do include payoffs, the authors \emph{make strong assumptions} to similarly ensure the constraint does not bind.\footnote{For example, \cite{dai2005maximum} assume that the network satisfies a so-called Extreme Allocation Available (EAA) condition, which ensures that the no-underflow constraint does not bind; \cite{stolyar2005maximizing} assumes that payoffs are generated only by the source nodes, which have infinite queue lengths.
	\cite{huang2011utility} consider networks where the payoffs are generated only by the output nodes, and show that a variant of backpressure avoids underflow entirely under this assumption.
	\cite{gurvich2014dynamic} assume that the network satisfies a so-called Dedicated Item (DI) condition.
	\yka{Add sentence about assumption in \cite{gurvich2014dynamic} here, since it is mentioned in the discussion.} \yka{mention EAA assumption in Dai and Lin as well.}}
In our setting, payoffs are essential (there is value generated by serving a customer), and so the constraint \emph{does} bind.

%For open queueing networks,
A machinery that introduces \emph{virtual queues} has been developed to extend backpressure to settings where the constraint binds; see, e.g., \cite{jiang2009stable}.
The main idea is to introduce a ``fake'' supply unit into the network each time the constraint binds, to preserve the SGD property of backpressure. In open queueing networks, these fake supply units eventually leave the system, and so have a small effect (under appropriate assumptions). In our closed network setting, these fake supply units, once created, never leave and so would build up in the system, leading to very poor performance. In Section \ref{subsec:underflow}, we provide a detailed discussion of the challenge posed by the no-underflow constraint, and how it prevents us from using backpressure as is.
%The challenge arises when backpressure recommends a decision

%\pq{In general, solving such stochastic control problems is difficult and requires substantial statistical knowledge of the underlying network randomness. The challenge stems from the \emph{no-underflow constraint} which couples the present and future decisions: as a physical constraint, each admission  needs to be backed by an available supply unit at the demand origin. Most of the existing approaches consider backpressure/MaxWeight policy and focus on \emph{open networks}. It is known that backpressure/MaxWeight policy is near-optimal if either: (i) The payoffs are not associated with control decisions \emph{per se} but with queue lengths; (ii) The network has special structure; or (iii) The system can send fake/null supply units when the demand origin runs out of supply. However, our case belongs to none of the above as we consider a closed network with general structure and control-associated payoffs. The null supply units would not help because unlike in open networks, they never leave the system once generated.}
%
%More detailed discussion in section 4.}
%
%The objective considered in this paper differs from previous work, which leads to a key challenge that we describe below.
%For instance, \cite{dai2005maximum,dai2008asymptotic} consider the objective of stabilizing the network and minimizing workload (i.e. a linear combination of queue lengths), and show that backpressure policy (BP) is asymptotically optimal for a class of problems where the BP allocation can always be achieved, i.e. they naturally do not use supply units from empty queues.
%
%In our case, however, the goal is to maximize payoff, which is determined by control decisions rather than queue lengths.
%With this new objective, in most of the problem instances BP allocation sometimes \emph{does} try to dispatch from empty queues, which makes the allocation infeasible and leads to difficulty.

%We will refer to this issue as the \textit{underflow problem}, as they come from the \emph{no-underflow constraint}: as a physical constraint, each admission decision needs to be backed by an available supply unit at the origin of demand.
%
%We refer to this challenge as the \textit{underflow problem}.
%The problem is further complicated by the fact that our model is \emph{multi-hop} where supply units circulate in the system, unlike traditional revenue management problems \citep[e.g., see][]{gallego1994optimal} and dynamic bipartite matching problems \citep[e.g.,][]{caldentey2009fcfs} where the network is \textit{one-hop}. In fact, the no-underflow constraint captures the tension between the payoff effect and queueing effect of admission decisions.



%It indicates that the state space has reflecting boundary \citep{chen1991stochastic,bramson2010positive}, which remains one of the main difficulties in dynamic scheduling of queueing systems.
%
\smallskip
\textbf{Our solution: Mirror Backpressure.}
In solving this problem, we introduce a novel class of policies which we call \emph{Mirror Backpressure}.
%, and show the power of this paradigm by obtaining an elegant solution to the ride-hailing control problem. % to address these issues.
MBP generalizes the celebrated backpressure (BP) policy  and is as simple and practical as BP. Whereas BP uses the queue lengths as congestion costs, MBP employs a flexibly chosen \emph{congestion function} to translate from queue lengths to congestion costs.
MBP features a simple and intuitive structure: for example, in the entry control setting, the platform admits a demand only if the payoff of serving it outweighs the difference between congestion costs at the destination and origin of the demand.
%The congestion cost is an increasing function of queue lengths.
Crucially, the congestion function is designed so that MBP has the property that it executes dual \emph{stochastic mirror descent} \citep{nemirovsky1983problem,beck2003mirror} on the platform's continuum limit optimization problem, with the chosen mirror map.\footnote{The special case of the congestion function being the identity function corresponds to standard BP, which has the property of executing stochastic gradient descent, a special case of mirror descent \citep{eryilmaz2007fair}.}
The mirror map can be flexibly chosen to fit the problem geometry arising from the no-underflow constraints. Roughly, we find better performance with congestion functions which are steep for small queue lengths, the intuition being that this makes MBP more aggressive in protecting the shortest queues (and hence preventing underflow). In case of finite buffers, we find it beneficial to use congestion functions which moreover increase  steeply as the queue length approaches buffer capacity, to prevent buffer overflow (Section~\ref{subsec:extend-barrier}).

We develop a general machinery to prove performance guarantees for MBP, which draws inspiration from two distinct toolkits: the machinery for proving convergence of mirror descent from the optimization literature, and the Lyapunov drift method from the network control literature. We provide a ready Lyapunov function for any MBP policy.
Furthermore, we improve upon the Lyapunov drift method to obtain a sharp bound on the suboptimality caused by the no-underflow constraint. Our analysis exploits the structure of the platform's continuum limit optimization problem in a novel way (see Section~\ref{sec:proof_sketch}). %: roughly, we leverage that larger payoffs accrue (on average) at times when estimated shadow prices are far from optimal.}
%This is in sharp contrast to much of the queueing literature, where finding a suitable problem-specific Lyapunov function has been quite an ``art form'' \citep[see, e.g.,][]{maguluri2016heavy}.

Our work fits into the broad literature on the control of stochastic processing networks \citep{harrison2000brownian}.  Our MBP methodology for designing blind control policies with provable guarantees applies to open queueing networks as well.
We are optimistic that MBP will prove broadly useful in the control of queueing networks.

\smallskip
\textbf{Main contributions.}
To summarize, we make two main contributions in this paper:
\begin{compactenum}[(i),wide, labelwidth=!, labelindent=0pt]
%\begin{enumerate}
	\item \textbf{Mirror Backpressure: a class of near-optimal control policies for queueing networks that are completely blind.}
	In general settings that consider entry control, pricing, and flexible assignment, we propose a family of dynamic control policies for queueing networks, the Mirror Backpressure policies, that have strong transient and steady state performance guarantees.
	The MBP policies are simple and practical, and do not require any prior knowledge of demand arrival rates (which are permitted to vary in time), making them promising for applications. Policy design boils down to choosing suitable congestion functions.
	%
	\item \textbf{A framework for systematic design and analysis of MBP control policies.}
	Our control framework has a tight connection with mirror descent, which makes the process of policy design and analysis both systematic and flexible, and allows us to handle the challenging no-underflow constraint.
	%(i) Design: The corresponding MBP policy is immediate from the choice of mirror map, which can be flexibly chosen to fit problem geometry.
	%(ii) Analysis:
	The general machinery we develop can be seamlessly leveraged to design policies with provable guarantees for a variety of settings.
	This is in contrast with various intricate approaches in the queueing literature that do not easily generalize.
	
	
	%Mirror Backpressure policies (implicitly) execute mirror descent on the controller's optimization problem, which allows problem geometry (no-underflow constraints) to be incorporated systematically in the design of the control policy. We are optimistic this will be the first of many problems in the control of queueing networks for which MBP will provide provably near optimal policies.
	%\yk{Rewrite this.}
	%We show that the MBP policy is closely connected to the stochastic mirror descent algorithm applied to a certain deterministic optimization problem.
	%	This connection makes it possible to apply analytical tools from optimization literature to our analysis.
	%	In particular, our proof is based on a novel and natural Lyapunov function, the Kullback-Leibler divergence, that arises from the mirror descent perspective.
	%	Our approach can also be seamlessly extended to incorporate dynamic pricing.
%\end{enumerate}
\end{compactenum}
\begin{comment}
(Vanilla) Backpressure (VBP) is very attractive as a simple and practical policy for state dependent control of queueing networks that does not require knowledge of demand arrival rates.
%
Roughly speaking, in entry control setting, VBP admits a demand if and only if the corresponding revenue outweigh the (normalized) queue length difference between the destination and origin.
%
The policy is semi-local, i.e. it only uses the queue length at the origin and destination.
%
However, VBP does not systematically incorporate no-underflow constraints, and no existing result (to the best of our knowledge) provides performance guarantee for VBP in our setting (see Section~\ref{subsec:lit-review}).
%
MBP generalizes VBP by replacing the queue length with a function of the queue length, and the choice of such functions can be guided by MBP's connection to mirror descent, leading to an interesting interplay between policy design and problem geometry.
\end{comment}

%In Section~\ref{sec:extension} we extend the main joint entry-assignment control (JEA) model and include pricing as control lever. 
%We study  in Section~\ref{subsec:jea} and joint pricing-assignment control (JPA) in Section~\ref{subsec:jpa}. 
%Our control policies and performance guarantees extend seamlessly.


%\subsection{Applications}\label{subsec:application}
\paragraph{Applications.} Our models (JEA in Section~\ref{sec:model} and JPA in Section~\ref{sec:extension}) include a number of key ingredients common to many applications.
We illustrate its versatility by discussing the application to shared transportation systems (Section~\ref{sec:shared-transportation}) and the application to scrip systems (Appendix~\ref{sec:scrip-systems}). These applications and the relevant settings in the paper are summarized in Table~\ref{tab:application_model}.

\begin{table}[htbp!]
	\small
	\centering
	\begin{tabular}{ccc}
		\toprule
		\emph{Application} & \emph{Control lever} & \emph{Corresponding setting in this paper} \\
		\midrule
		Ride-hailing in USA, Europe & Pricing \& Dispatch & Joint pricing-assignment\\
		%
		Ride-hailing in China & Admission \& Dispatch & Joint entry-assignment\\
		%
		%Ride-hailing& Dynamic pricing \& Dispatch & Pricing/Joint pricing-assignment \\
		%
		Bike sharing & Reward points & Pricing (finite buffer queues) \\
		%
		Scrip systems & Admission \& Provider selection   & Joint entry-assignment\\
		\bottomrule
	\end{tabular}
	\caption{Summary of applications of our model, the control levers therein and the corresponding settings in this paper.
		See %Sections \ref{sec:model} to \ref{sec:proof_sketch} for the entry control setting, and
Section~\ref{sec:model} for the joint entry-assignment and Section~\ref{sec:extension} for the joint pricing-assignment settings.
For each setting, we design MBP policies that are near optimal.
	}
	\label{tab:application_model}
\end{table}

Shared transportation systems include ride-hailing and bike sharing systems. Here the nodes in our model correspond to geographical locations, while supply units and demand units correspond to vehicles and customers, respectively. Bike sharing systems dynamically incentivize certain trips using point systems to minimize out-of-bike and out-of-dock events caused by demand imbalance. Our pricing setting is relevant for the design of a dynamic incentive program for bike sharing; in particular, it allows for a limited number of docks. Ride-hailing platforms make dynamic decisions to optimize their objectives (e.g., revenue, welfare, etc.). For ride-hailing, our pricing-assignment model is relevant  in regions such as North America, and our entry-assignment control model is relevant in in regions where dynamic pricing is undesirable like in China.
We perform realistic simulations of ride-hailing and find that our MBP policy, suitably adapted to account for positive travel times, performs well (Section~\ref{subsec:numerics-ridehailing}).


	A scrip system is a nonmonetary trade economy where agents use scrips (tokens, coupons, artificial currency) to exchange services (because
%	These systems are typically implemented when
monetary transfer is undesirable or impractical), e.g., for babysitting or kidney exchange.
	A key challenge in these markets is the design of the
admission-and-provider-selection rule:
	If an agent is running low on scrip balance, should they be allowed to request services? If yes, and if there are several possible providers for a trade, who should be selected as the service provider?
	In Appendix~\ref{sec:scrip-systems}, we show that a natural model of a scrip system is a special case of our entry-assignment control setting, yielding a near optimal admission-and-provider-selection control rule.




\subsection{Literature Review}
\label{subsec:lit-review}

\textbf{MaxWeight/backpressure policy.}
Backpressure \citep[also known as MaxWeight, see][]{tassiulas1992stability,georgiadis2006resource} are well-studied dynamic control policies in constrained queueing networks for workload minimization \citep{stolyar2004maxweight,dai2008asymptotic}, queue length minimization \citep{eryilmaz2012asymptotically} and utility maximization \citep{eryilmaz2007fair},  etc.
Attractive features of MaxWeight/backpressure policies include their simplicity and provably good performance, and that arrival/service rate information is not required beforehand. The main challenge  in using backpressure is the no-underflow constraints, as described earlier.
Most of this literature considers the open queueing networks setting, where packets/jobs enter and leave, and there is much less work on closed networks.
%
An exception is a recent paper on assignment control of closed networks by \citet*{banerjee2018SMW}, which shows the large deviations optimality of ``scaled'' MaxWeight policies. %/complete resource pooling (CRP)
Importantly, in that paper %the objective is throughput maximization, and
the demand arrival rates are assumed to satisfy a strong near balance assumption (``complete resource pooling''), as a result of which it suffices to consider non-idling policies (i.e., a ``greedy'' policy with assignment control only).
In the present paper, in contrast, %the objective is more general \emph{and}
we allow very general demand arrival rates, which makes it necessary to deploy idling policies (e.g., entry control, pricing) to achieve good performance. 
\pqr{again, do we want to shorten the discussion of SMW paper here? It is pretty long.}
Indeed, already under an illustrative model (Section~\ref{sec:model}) the CRP assumption of \citet*{banerjee2018SMW} is automatically violated; see Remark~\ref{rem:CRP-is-violated-and-greedy-is-suboptimal} in Section~\ref{sec:model}.
% and the greedy policy fails to achieve asymptotic optimality. \yka{Need to explain how in Section 2 that CRP is automatically violated.}
%

While previous works use queue lengths or their power as congestion costs \citep{stolyar2004maxweight}, our MBP policies significantly generalize backpressure by allowing a general increasing function (e.g., the logarithm) of queue lengths as congestion costs. As with backpressure, MBP policies carry provable guarantees. %Thus MBP is a significant generalization of backpressure.

\begin{comment}
\paragraph{No-underflow constraint in queueing control.} \yk{perhaps we can skip this paragraph entirely, since it is already covered?}
The no-underflow constraint of queue lengths is one of the main challenges in applying the backpressure methodology to general settings.
%the control of queueing systems \citep[see e.g.][for the diffculty of studying reflected process even in the limit.]{bramson2010positive,gamarnik2015stability}
%
\cite{dai2005maximum,dai2008asymptotic} consider a class of queueing control problems where the objective is throughput maximization or workload minimization, and there the no-underflow constraint does not bind for backpressure policies.
%However, when the objective becomes payoff maximization, backpressure policies violate no-underflow constraints for typical networks hence their argument does not apply to our problem.
%
\cite{stolyar2005maximizing,huang2011utility} consider the problems where either the source nodes or sink nodes of the network generate payoff, while the other nodes only process demands. The no-underflow constraint does not bind either.
%Comparing to these works, the no-underflow constraint is harder to handle in our case because each node can generate payoff as well as processing demands, and there is no source or sink since the network is closed.
%
\cite{jiang2009stable} use virtual queue based controls, which is difficult to analyze theoretically for finite systems and may fail entirely in our closed network setting, since the number of fake packets (created when dispatching from an empty queue) would grow without bound.
Our approach is systematic and provides a transient bound for finite systems.
\end{comment}

{
\textbf{Mirror Descent.} Mirror descent (MD) is a generalization of the gradient descent algorithm for optimization, which was proposed by \cite{nemirovsky1983problem}, see also \cite{beck2003mirror}. MD is much more flexible than gradient descent as one can freely choose a ``mirror map''  that captures the geometry of the problem (including its objective and its constraints).
Recently, there have been several works that use MD to solve online decision-making problems \citep[e.g.,][]{gupta2020interior}. Notably, \cite{bubeck2018k} uses MD to obtain an improved approximation factor for a worst-case version of the so-called ``$k$-server problem''; the $k$-server problem bears a certain resemblance to our setting in that the controller needs to manage the spatial distribution of supply.
A key difference between our work and the existing works is that our proposed simple control policies remarkably have the \emph{property} that they induce the queue lengths to follow MD dynamics, whereas the existing works actively run MD to solve their algorithmic problems.
}

\textbf{Applications: shared transportation, scrip systems.}
Most of the ride-hailing literature studied controls that require the exact knowledge of system parameters:
\citet{ozkan2016dynamic} studied payoff maximizing assignment control in an open queueing network model,
\citet{braverman2016empty} derived the optimal state independent routing policy that sends empty vehicles to under-supplied locations,
\citet*{banerjee2016pricing} adopted the Gordon-Newell closed queueing network model and considered various controls that maximize throughput, welfare or revenue.
%Our previous work
%which is shown to be much more effective in managing stochastic fluctuations in the system
\citet{balseiro2019dynamic} considered a dynamic programming based approach for dynamic pricing for a specific network of star structure. (\citet{ma2019spatio} studied the somewhat different issue of ensuring that drivers have the incentive to accept dispatches by setting prices which are sufficiently smooth in space and time, in a model with no demand stochasticity.)
\citet*{banerjee2018SMW} which assumes a near balance condition on demands and equal pickup costs may be the only paper in this space that does not require knowledge of system parameters.
%\yka{deleted `` which is shown to be much more effective in managing stochastic fluctuations in the system''. If exponentially fast convergence in $K$ is the notion of effectiveness then the reader will expect that we will obtain such convergence here. We should rather focus on how state independent policies need knowledge of system parameters.} despite the key advantage that state dependent control can yield near optimal performance even in the absence of knowledge about system parameters.
%
Comparing with \citet*{banerjee2016pricing} which obtains a steady state optimality gap of $O(\frac{1}{K})$ (in the absence of travel times) assuming \emph{perfect} knowledge of demand arrival rates which are assumed to be \emph{stationary}, our control policy achieves the same steady state optimality gap with \emph{no} knowledge of demand arrival rates, and further achieves a \emph{transient} optimality gap under \emph{time-varying} demand arrival rates of $O(\frac{K}{T} + \frac{1}{K} +\sqrt{\eta K})$ for a finite number of arrivals $T$ and average changes of up to $\eta$ per period (i.e., per arrival) in demand arrival rates. %The aforementioned works except \citet{ozkan2016dynamic}
Some of these papers are able to formally handle travel delays: \citet{braverman2016empty}, \citet{banerjee2016pricing}, and \citet*{banerjee2018SMW} prove theoretical results for the setting with i.i.d. geometric/exponential travel delays; \citet{ma2019spatio} consider deterministic travel delays. On the other hand, \citet{balseiro2019dynamic} ignores travel delays in their theory and later heuristically adapt their policy to accommodate travel delay (the present paper follows a similar approach). %\yk{please clarify briefly what the model of travel delays is for each of these papers. e.g., BFL, BKQ and Braverman et al allow iid geometric travel delays. What about Balseiro et al? This clarification can be placed in Sec 7.1.1 or else here. And will copy it in the response.}
On the other hand, \cite{ozkan2016dynamic} is the only paper among these  which (like the present paper) allows time-varying demand. %\yk{pending to do our extension to slowly time varying demand.}
%

Our model can be applied to the design of dynamic incentive programs for bike sharing systems \citep{chung2018bike} and service provider rules for scrip systems \citep{johnson2014analyzing,agarwal2019market}.
For example, the ``minimum scrip selection rule'' proposed in \cite{johnson2014analyzing} is a special case of our policy, and our methodology leads to control rules in much more general settings as described in Appendix~\ref{sec:scrip-systems}. %See Section \ref{subsec:application} for more discussion on these applications.



\yka{commented a bunch of stuff about scaling of previous results.}
%\cite{banerjee2016pricing} showed finite system bounds with an $O(1/{\N})$ stationary regret for a variety of objectives as $\N\to\infty$ in the absence of service times and an $O(1/\sqrt{\N})$ regret with service times, where $K$ is the number of cars.
%\cite{braverman2016empty} observed from simulation an $O(1/\sqrt{\N})$ stationary regret (of throughput) as $\N\to\infty$, \cite{banerjee2018SMW} proved $O(\exp(-\alpha\N))$ $(\alpha>0)$ stationary regret (of throughput).
%To the best of our knowledge, we are the first to provide a transient regret in this setting.
%Several recent works study pricing aspects of ride-hailing; see, e.g., \cite{adelman2007price,bimpikis2016spatial,waserhole2016pricing,cachon2017role,hall2015effects}.

\textbf{Other related work.}
A related stream of research studies online stochastic bipartite matching, see, e.g., \cite{caldentey2009fcfs,adan2012loss,buyic2015approximate,mairesse2016stability};
the main difference between their setting and ours is that we study a \emph{closed} system where supply units never enter or leave the system. Network revenue management is a classical set of (open network) dynamic resource allocation problems, e.g., see \cite{gallego1994optimal,talluri2006theory}, and recent works, e.g., \cite{bumpensanti2018re}.
\cite{jordan1995principles,desir2016sparse,shi2015process} and others study how process flexibility can facilitate improved performance, analogous to our use
of assignment control to maximize payoff (when all pickup costs are equal), but the focus there is more on network design than on control policies.
\yka{cite process flexibility, no? shi, wei, zhong could be our reviewers. same for weina wang.}
Again, this is an open network setting in that each supply unit can be used only once. %, in contrast to our closed setting.


\subsection{Organization of the Paper}
The remainder of our paper is organized as follows.
%We describe the connection to our motivating applications in Section \ref{subsec:application}.
%From Section \ref{sec:model} to Section \ref{sec:proof_sketch} we focus on the entry control setting as an illustrative example of our approach:
Section \ref{sec:model} presents our main model of joint entry-assignment control with time-varying demand arrival rates, and the platform objective.
Section \ref{sec:mbp} introduces the Mirror Backpressure policy and presents our main theoretical result, i.e., a performance guarantee for the MBP policies.
Section \ref{sec:static} introduces the static planning problem and describes the connection between the MBP policies and mirror descent.
Section \ref{sec:proof_sketch} outlines the proof of our main result.
In Section \ref{sec:extension}, we provide MBP policies for the joint pricing-assignment control setting, demonstrating the versatility of our approach.
In Sections~\ref{sec:shared-transportation} we discuss the applications to shared transportation systems.
% and scrip systems, respectively.
	%to scrip systems and describe a simulation study of MBP policies for ridehailing using NYC yellow cab data.}
%We conclude in Section \ref{sec:discuss} and discuss the future directions.

\textbf{Notation.} All vectors are column vectors if not specified otherwise.
The transpose of vector or matrix $\bx$ is denoted as $\bx^{\T}$.
We use $\boe_i$ to denote the $i$-th unit column vector with the $i$-th coordinate being $1$ and all other coordinates being $0$, and $\mathbf{1}$ ($\bzero$) to denote the all $1$ ($0$) column vector, where the dimension of the vector will be indicated in the superscript when it is not clear from the context.

\begin{comment}
Developed a \textbf{state-dependent pricing/assignment} policy in \textbf{general} setting for \textbf{closed} queueing networks.

\noindent\textbf{Technical Challenges:}
\begin{itemize}
\item Policy is \textit{idling}, i.e. the policy should tell us when to drop a demand.
\item So-called `underflow problem' in the scheduling of multi-hop networks \citep{huang2011utility}, i.e. queues supposed to be assigning supplies from go empty.
\end{itemize}

\noindent\textbf{Machinery:}
\begin{itemize}
\item Primal-dual view of back-pressure policy.
\item Non-asymptotic regret analysis of stochastic gradient descent (SGD) .
\end{itemize}

\noindent\textbf{Contribution:}
\begin{itemize}
\item Introduce the \textit{mirror back-pressure} policy that elegantly deals with underflow problem.
\item A simple, implementable policy with both transient and stationary horizon performance guarantee.
\item Bridging queueing and stochastic approximation algorithms, view queueing assignment problems as mini-batch SGD type algorithms.
\end{itemize}
\end{comment} 

==> 4-intuition.tex <==
\section{Intuition: the MBP Policies and Mirror Descent}\label{appen:md-intuition}

\yk{Isn't this section too long given that \cite{gupta2020interior} has already worked all this out? Even they spend less space on this, and that too in their appendix, right? I suggest to move most or all of the section to an appendix. What part is needed in the main paper? I suspect only the SPP, Prop 1, and the dual problem. That material can be incorporated in the proof section.}
In this section, we describe the main intuition behind the success of MBP policies, namely, that they execute (dual) mirror descent on certain deterministic optimization problems.
%
In Section \ref{subsec:fluid_problem}, we define a sequence of deterministic optimization problems which arise in the continuum limit: the \emph{static planning problem} ({SPP}), whose values we use to upper bound the optimal finite (and infinite) horizon per period $W^*_T$ (and $W^*$) defined in \eqref{eq:obj_finite} and \eqref{eq:obj_inf}.
%
In Section \ref{subsec:dual-SD-and-VBP}, we first review the interpretation of the celebrated Backpressure (BP) policy as a stochastic gradient descent algorithm on the dual of the SPP,
and then proceed to generalize the argument to informally show that MBP executes mirror descent on the dual of SPP.
%
In Section \ref{subsec:underflow} we discuss the main challenge in turning the intuition into a proof, namely, the no-underflow constraint.

\subsection{The Static Planning Problems}\label{subsec:fluid_problem}
We first introduce the linear programs (LP) that will be used to upper bound $W^*_T$ and $W^*$.
The LP, called the static planning problem (SPP) \citep[see, e.g.,][]{harrison2000brownian,dai2005maximum}, is defined for any demand arrival rates $\bphi$:
\begin{align}
\hspace{-0.2cm}\textup{SPP($\bphi$)}:\,\textup{maximize}_{\bx} \; &
\sum_{\tau\in \cT, j\in\mathcal{P}(\tau),k\in\mathcal{D}(\tau)}\ w_{j\tau k} \cdot \phi_{\tau} \cdot  x_{j\tau k}
\label{eq:fluid_obj}\\
\textup{s.t.}\; &
\sum_{\tau\in \cT, j\in\mathcal{P}(\tau),k\in\mathcal{D}(\tau)}\ \phi_{\tau}\cdot x_{j\tau k}(\boe_j - \boe_k) =\bzero
%
\hspace{2.8cm} \textup{(flow balance)} \label{eq:fluid_flow_bal}\\
%
&\sum_{j\in \mathcal{P}(\tau), k\in \mathcal{D}(\tau)}x_{j\tau k}\leq 1, \ x_{j\tau k} \geq 0\, ,  \, \forall j,k \in V,\ \tau\in\cT .
%
\hspace{0.1cm} \textup{(demand constraint)} \label{eq:fluid_dmd_constr}
\end{align}
%
One interprets $x_{j\tau k}$ as the fraction of type $\tau$ demand which is served by pickup location $j$ and dropoff location $k$, and the objective \eqref{eq:fluid_obj} as the rate at which payoff is generated under the fractions $\bx$.
In the SPP \eqref{eq:fluid_obj}-\eqref{eq:fluid_dmd_constr}, one maximizes the rate of payoff generation subject to the requirement that the average inflow of supply units to each node in $V$ must equal the outflow (constraint \eqref{eq:fluid_flow_bal}), and that $\bx$ are indeed fractions (constraint \eqref{eq:fluid_dmd_constr}).
%Constraint \eqref{eq:fluid_flow_bal} means that: ignoring stochastic fluctuations, for a policy to be feasible in the long run, the average inflow of supply units to each node in $V$ must equal the outflow.
%Constraint \eqref{eq:fluid_dmd_constr} follows from the definition of feasible policies given in Section \ref{sec:model}.
%Subject to these constraints, the policy is chosen to maximize the per period revenue generated.
%
Let $W^{\textup{SPP($\bphi$)}}$ be the optimal value of SPP($\bphi$).
The following proposition formalizes that, the optimal finite horizon per customer payoff $W^*_T$ cannot be much larger than $W^{\aspp}$ where $\bar{\bphi}\triangleq \frac{1}{T}\sum_{t=0}^{T-1}\bphi^t$.
%as is typical in such settings, $W^{\aspp}$ is an upper bound on the optimal steady state (per customer) payoff $W^*$ It further establishes that 
%
\begin{prop}\label{prop:fluid_ub}
	For any horizon $T<\infty$, any $K$ and any starting state $\bq[0]$, the finite horizon and steady state average payoff $W^*_T$, $W^*$ are upper bounded as
	\begin{align}\label{eq:fluid_ub}
		W^*_T \leq W^{\aspp} + m \frac{K}{T}\, ,\quad
		W^* \leq W^{\aspp}\, .
		%,\qquad W^* \leq \Wspp \, .
	\end{align}
	%where $w_{\max}\triangleq \max_{j,k\in V}|w_{jk}|$, $W^*$ is the optimal value of \eqref{eq:fluid_obj}-\eqref{eq:fluid_dmd_constr}.
\end{prop}
%The proposition formalizes that, as is typical in such settings, $\Wspp$ is an upper bound to the long run expected revenue $W^*$.
We obtain the finite horizon upper bound to $W^*_T$ in \eqref{eq:fluid_ub} by slightly relaxing the flow constraint \eqref{eq:fluid_flow_bal} to accommodate the fact that flow balance need not be exactly satisfied over a finite horizon. The proof is in Appendix \ref{appen:proof-of-fluid-ub}.


\subsection{MBP Executes Dual Stochastic Mirror Descent on SPP}
\label{subsec:dual-SD-and-VBP}

The BP policy and our proposed MBP policies are closely related to the (partial) dual of the SPP($\bphi^t$):
\begin{align}
	\textup{minimize}_{\by}\, g^t(\by),\quad
	&\textup{for }
	g^t(\by) \triangleq\;
	\sum_{\tau\in \cT}
	\phi_{\tau}^t \max_{j \in \cP(\tau), k \in \cD(\tau)}
	\left(
	w_{j\tau k} + y_j - y_k
	\right)^+\, .\label{eq:partial_dual}
\end{align}
%
where $(x)^+\triangleq\max\{0,x\}$.
Here $\by$ are the dual variables corresponding to the flow balance constraints \eqref{eq:fluid_flow_bal}, and have the interpretation of ``congestion costs'' \citep{neely2010stochastic}, i.e., $y_j$ can be thought of as the ``cost'' of having one extra supply unit at node $j$.

In the rest of this subsection, we informally describe the interpretation of BP as stochastic gradient descent, and the interpretation of MBP as stochastic mirror descent, on problem \eqref{eq:partial_dual}.
%By definition, the demand constraint \eqref{eq:fluid_dmd_constr} is satisfied at any time by any admissible policy.
%However, the flow balance constraint \eqref{eq:fluid_flow_bal} only need to hold for the time average of $\bx[t]$, and can be violated at a particular time.
%To make sure flow balance is satisfied in the long run, we introduce Lagrange multipliers $\by\in\mathbb{R}^m$ for \eqref{eq:fluid_flow_bal} and derive the partial dual problem of \eqref{eq:fluid_obj}-\eqref{eq:fluid_dmd_constr}:
%


\textbf{Review of the interpretation of BP as dual stochastic subgradient descent.} Rich dividends have been obtained by treating the (properly scaled) current queue lengths $\bq$ as the dual variables $\by$, resulting in the celebrated backpressure (BP, also known as MaxWeight) control policy, introduced by  \citet{tassiulas1992stability}\pqa{Note to self: There is a citation formatting problem, which I fixed for Nicholson submissions, etc, but not this version.}, see also, e.g., \cite{stolyar2005maximizing,eryilmaz2007fair}. %, and shown to minimize delay and workload in open queueing networks \yk{can add citations, but try to avoid redundancy between here and related work}.
%We henceforth refer to this policy as Vanilla Backpressure (VBP).
Formally, BP sets the current value of $\by$ to be proportional to the current normalized queue lengths, i.e., $\by[t] = c\cdot\bar{\bq}[t]$ for some $\bar{\bq} \in \Omega$ defined, e.g., as in \eqref{eq:normalized_queue}, and some $c> 0$ and greedily maximizes the inner problem in \eqref{eq:partial_dual} %\yk{but the inner problem has disappeared from \eqref{eq:partial_dual}! I think we should show it there before giving the simplified expression, no?}
for every origin $j$ and destination $k$, i.e.,
\begin{align}
x_{j^*\tau k^*}^{\textup{BP}}[t]=
\left\{
\begin{array}{ll}
1 & \textup{ if } (j^*,k^*)=\textup{argmax}_{j\in\cP(\tau),k\in\cD(\tau)}w_{j\tau k} +
c \bar{q}_j[t] - c \bar{q}_k[t]\geq 0\textup{ and }q_j[t]>0\, ,\\
0 & \textup{ otherwise}\, .
\end{array}
\right.
\label{eq:VBP-defn}
\end{align}
%It is worth noting that $(\bw + \bR^{\T}\by)\circ \tilde{\bphi}$ is the \textit{reduced cost} in linear programming \citep[see, e.g.,][]{bertsimas1997introduction}.
The main attractive feature of this policy is that it is extremely simple and does not need to know demand arrival rates $\{\bphi^t\}$.
%We will point out the problem with VBP in our setting in Section \ref{subsec:underflow}, which motivates our novel generalization of backpressure to MBP.
The BP policy can be viewed as a \textit{stochastic subgradient descent (SGD)} algorithm on the dual problem \eqref{eq:partial_dual}, when the current state is in the \textit{interior} of the state space, i.e., when $q_j>0$ for all $j\in V$ \citep{huang2009delay}.
%Next, observe from \eqref{eq:bq-updates} that under any policy, we have
%\begin{align}
%	\bar{\bq}(t+1) = \bar{\bq}(t) - \frac{1}{K}\bR(\tilde{\ba}\circ\bx(t))\, .
%\label{eq:qdot}
%\end{align}
%since $\bR(\tilde{\ba}\circ\bx(t))$ is the mass of supply leaving each node in $V_S$ at time $t$.
To see this, denote the subdifferential (set of subgradients) of function $g^t(\cdot)$ at $\by$ as $\partial g^t(\by)$.
Observe that \emph{the expected change of queue lengths under BP is proportional to the negative of a subgradient of $g^t(\cdot)$ at $\by = c\cdot\bar{\bq}[t]$}, in particular %\yk{we should drop \eqref{eq:qdot}. \eqref{eq:bq-updates} suffices. I'll make the edit later.}
\begin{align}
\hspace{-0.2cm}-\frac{\tK}{c} \mathbb{E}[\by[t+1]-\by[t]]
= - \mathbb{E}[\bq[t+1] -\bq[t] ]=
\sum_{\tau \in \cT}\phi_{\tau}\sum_{j\in\cP(\tau),k\in\cD(\tau)}
x_{j\tau k}^{\textup{BP}}[t](\boe_j - \boe_k)
\in\partial g^t(\by[t])
\label{eq:subgrad-VBP}\, ,
\end{align}
where the first equality follows from the definition $\by[t]= c\cdot\bar{\bq}[t]$ (and the definition of normalized queue length \eqref{eq:normalized_queue}) and second equality is just the expectation of the system dynamics \eqref{eq:system-dynamics-jea}. Here $\sum_{\tau \in \cT}\phi_{\tau}\sum_{j\in\cP(\tau),k\in\cD(\tau)}
x_{j\tau k}^{\textup{BP}}[t](\boe_j - \boe_k)
\ \in\ \partial g^t(\by[t])$ follows from direct observation.
%since $g$ is a maximum of linear functions  of $\by$ parameterized by $\bx$, hence $g$ is convex and the gradient of a linear function among these which is an argmax at $\by[t]$ (in particular, the linear function parameterized by $\bx^{\textup{BP}}[t]$) is a subgradient of $g$ at $\by[t]$.

Eq. \eqref{eq:subgrad-VBP} shows that the evolution of $\by[t]$ when $\bq[t]>0$ is exactly an iteration of SGD with step size $\frac{c}{\tK}$.
%It is easy to verify that \yk{This is true only for $y = q(t)$.}
%\begin{align*}
%\bR(\tilde{\bphi}\circ \bx^{\textup{VBP}}(t)) \in \partial g(\by) \, .
%\end{align*}
%Also, defining the dual variable at the $t$-th time slot by $\by(t) \triangleq \bar{\bq}(t)$, observe that under the VBP policy, we have
%\begin{align}
%	\by(t+1) = \by(t) - \frac{1}{K}\bR(\tilde{\ba}\circ\bx^{\textup{VBP}}(t))\, ,\label{eq:vbp_subgrad}
%\end{align}
%since $\bR(\tilde{\ba}\circ\bx^{\textup{VBP}}(t))$ is the mass of supply leaving each node in $V_S$ at time $t$.
%Since $\mathbb{E}[\bR(\tilde{\ba}\circ\bx^{\textup{VBP}}(t))] = \bR(\tilde{\bphi}\circ\bx^{\textup{VBP}}(t))
%\in \partial g(\by(t))$, \eqref{eq:vbp_subgrad} is exactly an iteration of stochastic subgradient descent with step size $\frac{1}{K}$.
This interpretation of BP as stochastic subgradient descent leads to desirable properties including stability, approximate minimization of delay/workload, and approximate revenue maximization in certain networks \citep[see, e.g.,][etc.]{georgiadis2006resource}.\yka{please refine the prior sentence. you mean approximate/asymptotic minimization or maximization, right?}
%
However, as we will see in Section \ref{subsec:underflow}, in our setting the SGD property of backpressure breaks on the \emph{boundary} of state space, i.e., when there exists $j'\in V$ such that $q_{j'}=0$, due to the \emph{no-underflow} constraints $\bq\geq\bzero$.


\textbf{MBP executes dual stochastic mirror descent on the SPP.} The key innovation of our approach is to design a family of policies generalizing BP (MBP given in Algorithm \ref{alg:mirror_bp}) that \emph{executes stochastic mirror descent on the partial dual problem \eqref{eq:partial_dual} (with flow constraints dualized), with $\nq[t]$ given by \eqref{eq:normalized_queue} being the mirror point and the inverse mirror map being the (vector) congestion function $\mathbf{f}(\nq)\triangleq [f(\bar{q}_1),\cdots,f(\bar{q}_m)]^{\T}$.}
Mathematically, if $\bq>0$, we have
%The queue lengths constitute the mirror point.
\begin{align}
%-\tilde{K}\mathbb{E}[\nq[t+1]-\nq[t]] =
  - \mathbb{E}[\bq[t+1] -\bq[t] ]=
\sum_{\tau \in \cT}\phi_{\tau}\sum_{j\in\cP(\tau),k\in\cD(\tau)}
x_{j\tau k}^{\textup{MBP}}[t](\boe_j - \boe_k)
 \in \partial g^t(\by) \Big |_{\by = \bof(\bar{\bq}[t])}
\label{eq:subgrad-MBP}\, ,
\end{align}
%
where $\bx^{\textup{MBP}}[t]$ is the control defined in Algorithm \ref{alg:mirror_bp}; notice that the entry rule $\bx^{\textup{MBP}}[t]$ has the same form as that for BP \eqref{eq:VBP-defn} except that it uses a general congestion function $f(\bar{q}_j)$, leading to \eqref{eq:subgrad-MBP} for MBP via the same reasoning that led to \eqref{eq:subgrad-VBP} for BP.
Thus, MBP performs stochastic mirror descent on the partial dual problem \eqref{eq:partial_dual}, which generalizes the previously known fact that BP performs stochastic gradient descent.
%
A main advantage of mirror descent over gradient descent is that it can better capture the geometry of the state space via an appropriate choice of mirror map \citep[see, e.g.,][]{beck2003mirror}.
%
%The analysis of mirror descent is almost completely parallel to that of gradient descent: they both rely on Lyapunov functions, which represents the proximity between current variables and the set of their optimal values.
%The difference lies in the choice of Lyapunov functions: for gradient descent, squared Euclidean distance is often used as the proximity measure; for mirror descent, the Bregman divergence determined by the mirror map is used (e.g., the Kullback-Leibler divergence is the Lyapunov function for the exponential mirror map $q_j=e^{y_j} \, \Leftrightarrow \, y_j = f(q_j) = \log q_j$, i.e., for the logarithm congestion function, see Remark \ref{rem:general_mirror_map}).
In our setting, the congestion function $\mathbf{f}(\nq)$ is the inverse mirror map and can be flexibly chosen.

Our approach blending backpressure and mirror descent with a flexibly chosen mirror map is novel.
We believe it can serve as a general framework for systematic design of provably near optimal backpressure-like control policies for queueing networks in settings with hairy practical constraints.


\subsection{Challenge: No-underflow Constraints}\label{subsec:underflow}

As we have discussed earlier, the no-underflow constraints pose a challenge when applying backpressure to various settings.
\pq{In this section, we provide a detailed discussion on: (i) Why BP might fail in dealing with no-underflow constraints; (ii) The existing algorithms that cope with no-underflow constraints; and (iii) Why MBP could alleviate the underflow problem.}

\yk{Maybe this part can go in the same appendix where the example showing the failure of BP is?}
\pq{\textbf{Why BP might fail in dealing with no-underflow constraints.}  Recall that BP uses a linear function of normalized queue lengths, i.e., $\by[t] = c\cdot \bar{\bq}[t]$ (where $c>0$), as shadow prices.
Intuitively, this could cause issues since $\bar{\bq}$ is subject to (physical) state space constraints, but the shadow prices $\bar{\by}$ can take any value since they are the Lagrange multipliers of equality constraints \eqref{eq:fluid_flow_bal}. Indeed, in Appendix \ref{append:subsec:bp_fails} we construct an example such that for all $\bar{\bq} \in \Omega$, the corresponding shadow prices $c\cdot \bar{\bq}$ are suboptimal for the dual problem \eqref{eq:partial_dual}.

Even if there are optimal dual variables $\by^*$ which correspond to a queue length vector, i.e., $\by^* = c\cdot \nq$ for some $\nq\in\Omega$, we construct an example in Appendix \ref{append:subsec:bp_fails} where the existing analysis of BP still fails. 
This is because in the analysis of BP one needs to show that the Lyapunov function decreases in expectation in each period, which roughly means that the queue lengths are ``pushed'' towards the interior of state space under BP. However, in our example we show that the Lyapunov drift could be positive at certain states due to underflow constraints.
}

\bigskip
\yk{\cite{gupta2020interior} have created a custom non-quadratic Lyapunov function to deal with both the no underflow constraint in their setting, and the setting in bin packing where linear space wastage is unavoidable (this is a different type of geometrical requirement). You have adapted their approach to the geometry of your problem, which is great. Why bother explaining in so much detail why DMW, PMW etc. do not work? (The underlying reason can be mentioned in the literature review itself and that should suffice to answer the request of ref 3 to compare to these works. I don't see the ref asking for a detailed comparison, right?)  In the end, one of the existing approaches in the literature does work once you pick the right non-linear function. (Their original arxiv version https://arxiv.org/pdf/1211.2687.pdf goes back to 2012, and describes the philosophy for a general ``congestion function'' though they don't call it by that name. Other folks may have done similar things before.)}

\pq{\textbf{Existing algorithms that deal with no-underflow constraints.} Notably, the works by \cite{jiang2009stable} and \cite{huang2011utility} both propose BP-type policies that cope with no-underflow constraints.
%
Specifically, \cite{jiang2009stable} introduce Deficit MaxWeight (DMW) policies where the decisions are based on virtual queues instead of physical ones as in BP. 
Virtual queues are almost the same as physical queues, with the crucial difference that they ignore the no-underflow constraints.
DMW sends ``null units'' when the assigned (dispatch) location runs out of supply units. By bounding the difference between the virtual queue process and the physical queue process (augmented with null units), they show that DMW is near-optimal. 
However, we cannot apply DMW to our closed network setting: In open queueing networks, these fake supply units eventually leave the system, and so have a small effect (under appropriate assumptions). In our closed network setting, these fake supply units, once created, never leave and so would build up in the system, irreparably damaging performance.

\cite{huang2011utility} propose Perturbed MaxWeight (PMW) policies which use affine functions $\by = c\cdot (\nq - \boldsymbol{\theta})$, instead of linear functions $c\cdot \nq$ as in BP, as shadow prices. 
For a specific family of open queueing networks (``networks with output reward''), they show that PMW is near optimal for certain choices of $\boldsymbol{\theta}$. 
We cannot apply PMW to our closed network setting because the analysis in \cite{huang2011utility} relies on network properties such as acyclicity, which the closed networks do not possess.
}

\bigskip
\yk{The below para can be incorporated in the next section, right? I'm aiming to eliminate the current section 4.}
\pq{\textbf{Why MBP alleviates the underflow problem.}
As mentioned earlier, BP could run into two issues due to the underflow constraints: (i) The queue lengths corresponding to the optimal dual variables lie outside of the state space; (ii) The Lyapunov drift could be positive at certain ``boundary states'', i.e., states where some of the queues are empty.

In the following analysis, we show that the underflow problem is provably alleviated by MBP policies with an appropriately chosen congestion function. We provide some high-level intuitions below.
%
Consider the MBP policy with congestion function $\bof(\cdot)$ given in \eqref{eq:inv_sqrt_mirror_map} and normalized queue lengths $\nq$ defined in \eqref{eq:normalized_queue}.
For issue (i), note that while the range of normalized queue length $\bar{\bq}$ belongs to $[0,1]$, the range of $f(\nq)$ goes to $(-\infty,-\sqrt{m})$ as $K\to\infty$. As a result, we can ensure that for large enough $K$, we can always find $\nq\in\Omega$ such that $\bof(\nq)$ corresponds to the optimal dual variable.\footnote{Note that optimal dual variables for \eqref{eq:partial_dual} is non-unique, since if $\by^*$ is optimal, $\by^* + \theta\mathbf{1}$ is also optimal for any $\theta\in\mathbb{R}$. Therefore we can always find an optimal dual variable that corresponds to $\bof(\nq)$ where $\nq\in\Omega$.}
For issue (ii), first note that this problem only occurs when there exists empty queues. 
At these states, the dual-suboptimality at $\bof(\nq)$ is large because $f(0)\to -\infty$ as $K\to\infty$, which creates a negative Lyapunov drift that ``pushes'' $\bof(\nq)$ towards the optimal dual variable. 
We formalize this observation in the next section. 
This corresponds to the intuition that MBP is more aggressive in preserving supply units in near-empty queues compared to BP, making the system less likely to violate the no-underflow constraints.
}



%

%Besides carrying formal guarantees, the MBP policy also achieves better performance than BP in simulations (Section \ref{subsec:numerics-ridehailing} and Appendix~\ref{appen:subsec:numerics-ridehailing}).




%\smallskip



\begin{comment}
\paragraph{One way to understand the difficulty caused by no-underflow constraints: \emph{reflecting boundaries}.}
The system state is constrained to be non-negative, hence when some of the queues become empty, the allocation corresponding to the subgradient descent direction can be infeasible.
%
Therefore the system state dynamics under BP is the ``reflected'' subgradient dynamics, where reflection happens on the boundary of state space $\Omega^K$ \citep[see, e.g.,][]{chen1991stochastic}.
%
It is well-known in the queueing literature that in general, directly analyzing the reflected process (the system state under BP in our case) is challenging, even if the original process is as simple as a Brownian motion with drift \citep[see, e.g.,][]{bramson2010positive,gamarnik2015stability}.

\paragraph{Existing approaches.}
Another example is where the network has certain structures, i.e. payoffs are only generated at source nodes \citep{stolyar2005maximizing} or sink nodes \citep{huang2011utility}.
For open networks, there are also variants of BP that deal with the underflow problem, for example, sending fake/null supply units when a node runs out of supplies \citep{huang2009delay}.

Our model does not fit into either of the above cases because the payoffs are directly generated by controls and the network structure is general.
The hack also does not work for our setting, because
the system will be overwhelmed by fake supply units as unlike in open networks, the fake supply units never leave the system once generated.

As discussed in Section \ref{sec:intro}, the existing results for BP rely on special structures of the models of consideration, but unfortunately, none of these approaches apply to our closed network setting, where the objective is payoff maximization.
\end{comment}

%
%Using a novel argument, we also show that VBP can be asymptotic optimal as well, provided that

%This challenge naturally raises the question of whether VBP is asymptotically optimal in our setting.
%
%However, a more interesting question would be, are there policies that inherit the advantages of VBP, while systematically deal with the underflow constraints?
%
%In the next section we provide an affirmative answer to the latter question, via an elegant approach related to the mirror descent algorithm.
%present an elegant and\yka{replaced ``unified'' with ``systematic''} systematic approach to address the no-underflow constraints via the mirror descent algorithm.


\begin{comment}
In particular, we have the following counterexample:
\begin{prop}
\textcolor{red}{for a fixed VBP policy, there exist a problem instance such that as $K\to\infty$, there is still non-trivial optimality gap.}
\end{prop}

\textcolor{red}{(A short explanation below, instead of a whole page, to give an idea why VBP sometimes does not work.)}
\paragraph{Problem 1: The dual optimum may lie outside the positive orthant.} The first problem is that the relevant dual optimum may not be in the positive orthant, and so $\bbq(t)$ cannot get close to it. Note that one of our flow constraints is redundant (flow balance at any $m-1$ nodes automatically implies flow balance at the remaining node), and correspondingly, $g(\by)$ is unchanged if all the $y_i$s are translated by the same amount,
i.e.,
\begin{align}
g(\by + \xi \mathbf{1}) = g(\by) \quad \forall \by \in \reals^m, \xi \in \reals \, .
\label{eq:g-translation-invariant}
\end{align} %i.e., $g(\by + \xi \mathbf{1}) = g(\by) \; \forall y \in \reals^m, \xi \in \reals$.
As a result the dual problem \eqref{eq:partial_dual} has a \emph{family} of optima resulting from translating any optimum.
Since for closed queueing networks we have $\sum_{i \in V_S}\bar{q}_i=1$,
the proxy dual variables $\nq(t)$ will converge to a member of the family of optimal $\by$ which satisfies $\sum_{i \in V_S} y_i = 1$.
However, this particular optimum lies \emph{outside} the positive orthant in a large class of instances.
\append{See Appendix \ref{append:dual_outside_pos_orthant} for such an example.}
In any such instance, the proxy dual variables $\bar{\bq}(t)$ under the VBP policy cannot approach a dual optimum and hence the payoff under the VBP policy does not achieve the upper bound even asymptotically (the long run per  period payoff is bounded away from $\Wopt$ even for $K \rightarrow \infty$). %\yk{A simple example can help. It can be in the appendix if needed.}
A possible solution is to ensure that $\bar{\bq}$ corresponding to the dual optimum lies in the positive orthant by interpreting a suitable translation $\bar{q}_i(t)-\zeta_i$ as the corresponding dual variable \citep{huang2011utility}, but then choosing an appropriate translation $\pmb{\zeta}$ would depend upon adequate knowledge of the demand arrival rates $\bphi$. Even if such knowledge is available, analysis of the VBP policy is complicated by another issue, which we describe next.
%:On the \textit{boundary} of the state space (i.e., when some queues are empty), however, the VBP policy suffers from so-called \textit{underflow problem} that could severely impact system performance. We will discuss this phenomenon in the next section.
%


\noindent\paragraph{Problem 2: Supply externalities and underflow.}
The analysis is complicated by the non-negativity constraint of queue lengths: the number of supply units assigned from a location cannot exceed the number of supply units available there.
As a result, the intended assignment \eqref{eq:vbp_subgrad} in each time slot might only be partially fulfilled, and the realized update is
%\begin{align}
%\by(t+1) = \by(t) - \frac{1}{K}\bR(\tilde{\ba}\circ\bx^{\textup{VBP}}(t) - \bu(t)) \, ,\label{eq:vbp_subgrad_bd}
%\end{align}
%where
%\begin{align*}
%\bu(t)
%=
% K\left[\frac{1}{K}[\bR]^+(\tilde{\ba}\circ\bx^{\textup{VBP}}(t))
% -
% \by(t)\right]^+ \geq \bzero\, .
%\end{align*}
\begin{align}
\by(t+1) &= \by(t) - \frac{1}{K}\bR(\tilde{\ba}\circ\bx^{\textup{VBP}}(t)) + \bu(t) \, ,\label{eq:vbp_subgrad_bd}
\end{align}
where $\bu(t)$ accounts for: (i) supplies that would be dispatched if the dispatched queue was non-empty; (ii) supplies that would arrive if the dispatched upstream queue was non-empty.

In some applications, VBP has provably good performance despite such boundary behavior.
For example, when the system is a one-hop network (i.e., the input-output matrix $\bR$ does not have negative entries), iteration \eqref{eq:vbp_subgrad_bd} is a \textit{projected SGD} step
\begin{align*}
\by(t+1) = \mathcal{P}_{\mathbb{R}^m_{+}}\left(\by(t) - \frac{1}{K}\bR(\ba\circ\bx^{\textup{VBP}}(t) )\right) \, ,
\end{align*}
here $\mathcal{P}_{\mathcal{S}}(\cdot)$ is the Euclidean projection onto set $\mathcal{S}$.

In multi-hop settings such as ride-hailing, iteration \eqref{eq:vbp_subgrad_bd} is \textit{not} a projected SGD step due to the existence of \textit{supply externalities}: \textit{starvation of upstream supply nodes (the dispatch location in ride-hailing) can affect supply availability at downstream supply nodes (the customer destination in ride-hailing)}.
Many works in the literature indirectly approach this problem by sending ``null units'' when the assigned (dispatch) location runs out of supply units \citep[see, e.g.,][]{huang2009delay}.
In our closed queueing network setting, however, this approach is not an option because  ``null supplies'' will gradually replace regular supplies since they never leave the system. The virtual queues approach \citep[see, e.g.,][]{stolyar2005maximizing} would seem to suffer from the same issue.
There are a small number of works that directly address no-underflow constraints, e.g., by considering a ``perturbed'' backpressure policy that keeps the queue lengths away from zero \citep[e.g.,][]{huang2011utility}.
The main drawback of this approach is that its parameters need to carefully chosen.
\end{comment}


%\textcolor{red}{\textbf{It would be sweet if we can put a simple instable counter-example here.}}
%for \textit{finite} $T$.

\begin{comment}
\begin{prop}\label{prop:fluid_upper_bound}
For any horizon $T< \infty$, any  $K$ and any starting state $\bq(0)$, the expected payoff generated by any policy $\pi\in\mathcal{U}$ is upper bounded as %$\Wopt_T \geq $ for any $\bq(0)$ and any $\pi$. Moreover $\Wopt_T$ is itself bounded above in terms of the value of the static fluid problem as
\begin{align}
\bar{v}^\pi(T) \leq \Wopt + \frac{(m-1)w_{\max} K}{T} \, ,
\label{eq:barv-ub}
\end{align}
where $\Wopt$ is the value of the static fluid problem.
In particular, the long run payoff under any policy $\pi\in\mathcal{U}$ is bounded above as $\limsup_{T \to \infty}\bar{v}^\pi(T) \leq \Wopt$.
\end{prop}
%\begin{proof}
\append{The proof is in Appendix \ref{append:fluid_ub}.}
%\end{proof}

The idea behind Proposition~\ref{prop:fluid_upper_bound} is as follows. As is typical in such settings, $\Wopt$ is an upper bound to the long run expected payoff. We obtain a \emph{finite horizon} upper bound in addition by slightly relaxing the flow constraint \eqref{eq:flow_balance_matrix} in the static fluid problem to
\begin{align}
\big |\mathbf{1}_S^T \bR(\btphi\circ\bx)\big | \leq \frac{K}{T} \qquad \forall \; S \subset V_S \, ,

\end{align}
where $\mathbf{1}_S$ is the vector with 1s at nodes in $S$ and $0$s at all other nodes.
In words, constraint \eqref{eq:approx_flow_balance} requires that for any subset $S$ of supply nodes, the magnitude of net per period flow into $S$ should not exceed $K/T$, i.e., over $T$ periods the net movement of supply into or out of $S$ should not exceed $K$. Clearly this constraint must hold since there are only $K$ supply units circulating in the system. Call the optimization problem defined by \eqref{eq:static_problem_matrix}, \eqref{eq:approx_flow_balance} and \eqref{eq:demand_constraint_matrix} the \emph{finite horizon fluid problem}, and denote its value by $\Wopt_T$. The proof of Proposition~\ref{prop:fluid_upper_bound} has to two key components. First we show that $\Wopt_T$ is an upper bound on the expected payoff over horizon $T$ under any policy. Second, we show that $\Wopt_T \leq \Wopt + \frac{(m-1)w_{\max}K}{T}$ by decomposing any feasible $\bx$ for the finite horizon fluid problem into a circulation (feasible for the static fluid problem) plus a directed acyclic flow with at most $K/T$ flow crossing any cut. Combining we get the proposition. % containing an upper bound on the finite horizon expected payoff under any policy.
content...
\end{comment} 

==> applications-backup.tex <==
\subsection{Applications}\label{subsec:application}
In Section \ref{sec:extension} we generalize the baseline model (which allows entry control only) and include pricing and flexible assignment as control levers. Our general model includes a number of key ingredients common to many applications.
We illustrate its versatility with the following applications, which are also summarized in Table \ref{tab:application_model}.
In Section~\ref{sec:scrip-systems} we discuss in detail the application to scrip systems (Item 3 below).
\pqr{In Sections~\ref{sec:sims} and \ref{sec:scrip-systems} we discuss the applications to ride-hailing and scrip systems, respectively.}

%\begin{enumerate}
\begin{compactenum}[(1),wide, labelwidth=!, labelindent=0pt]
	\item \emph{Online control of ride-hailing platforms.}
	Ride-hailing platforms make dynamic decisions to optimize their objectives (e.g., revenue, welfare, etc.).
	%
	Here the nodes in the model correspond to geographical locations, while supply units and demand units correspond to cars and customers, respectively.
	%
	For most ride-hailing platforms in North America, pricing is used to modulate demand, which we capture by the pricing model we will introduce in\footnote{Our model there is similar to that of \cite{banerjee2016pricing}, except that the platform does \emph{not} know demand arrival rates and we allow a finite horizon.}  Section~\ref{sec:extension}.
	%
	In certain countries such as China, however, pricing is a less acceptable lever, hence admission control of customers is used as a control lever instead.
	This corresponds to the entry control model described above. %\footnote{Some countries are halfway between the two approaches, e.g. India.}
	%
	In both cases, the platform can also decide where (near the demand's origin) to dispatch a car from, and where (near the demand's destination) to drop off a customer.
	These scenarios are well captured by the joint entry-assignment (JEA) and joint pricing-assignment (JPA) models to be introduced in Section \ref{sec:extension}.
	%
	%These decisions are made in an online manner based on the current/historical system configurations.
	%Our model of entry-control described above and joint entry-assignment control introduced later can be applied to this problem.
	%
	%\item \emph{Online control of ride-hailing platforms with pricing.}
	%For most ride-hailing platforms in North America, pricing are used to modulate demand.
	%The platform can also apply other control levers such as choosing where the dispatch a car, and dropping customers at locations near (but not exactly at) their destination.
	%The platform's objective can be revenue/welfare maximization etc.
	%(\citealt{banerjee2016pricing} considered the static control in this setting.)
	%The pricing and joint-pricing assignment setting of our model can be applied to this problem.
	%
	\item \emph{Dynamic incentive program for bike-sharing systems.}
	A major challenge faced by bike-sharing systems such as Citi Bike in New York City is the frequent out-of-bike and out-of-dock events caused by demand imbalance.
	One popular solution is to dynamically incentivize certain trips by awarding points (with cash value) depending on a trip's pickup and dropoff locations \citep{chung2018bike}.
	The optimal design of a dynamic incentive program corresponds to the pricing setting of our model. As we briefly discuss in Section \ref{sec:extension}\yka{I suggest to add a short note to Section 6 which describes how to deal with the constraint on number of docks/finite buffer sizes.}, a simple adaptation of our control methodology allows us seamlessly handle the additional constraints in a docked bikesharing system that there are only a certain number of docks at each location. %\yk{need to add an appendix and a pointer to it here.}
	%
	\item \emph{Scrip systems.}
	A scrip system is a nonmonetary trade economy where agents use scrips (tokens, coupons, artificial currency) to exchange services.
	These systems are typically implemented when monetary transfer is undesirable or impractical.
	For example, \cite{agarwal2019market} suggest that in kidney exchange, to align the incentives of hospitals, the exchange should deploy a scrip system that awards points to hospitals that submit donor-patient pairs to the central exchange, and deducts points from hospitals that conduct transplantations.
	Another well-known example is Capitol Hill Babysitting Co-op \citep[][see also \citealt{johnson2014analyzing}]{sweeney1977monetary}, where married couples pay for babysitting services by another couples with scrips.
	A key challenge in these markets is the design of the service provider selection rule:
	When there are several possible providers for a trade, who should be selected for service? If an agent is running low on scrip balance, should they be allowed to request services?
	We postpone the detailed discussion of how our model can facilitate the design of a near optimal provider selection rule to \pq{Section}~\ref{sec:scrip-systems}.
	%The joint entry-assignment setting of our model can address this problem: the agents can be viewed as nodes, scrips are supply units, and service requests are demands.
	%A graph structure of the nodes can capture the service compatibility between agents.
%\end{enumerate}
\end{compactenum}

\begin{table}[htbp!]
	\small
	\centering
	\begin{tabular}{ccc}
		\toprule
		\emph{Application} & \emph{Control lever} & \emph{Corresponding setting in this paper} \\
		\midrule
		Ride-hailing in USA, Europe & Pricing \& Dispatch & Joint pricing-assignment\\
		%
		Ride-hailing in China & Admission \& Dispatch & Joint entry-assignment\\
		%
		%Ride-hailing& Dynamic pricing \& Dispatch & Pricing/Joint pricing-assignment \\
		%
		Bike-sharing & Reward points & Pricing (finite buffer queues) \\
		%
		Scrip system & Provider selection   & Joint entry-assignment (Appendix~\ref{sec:scrip-systems})\\
		\bottomrule
	\end{tabular}
	\caption{Summary of applications of our model, the control levers therein and the corresponding settings in this paper.
		See Sections \ref{sec:model} to \ref{sec:static} for the entry control setting, and Section \ref{sec:extension} for other settings.
		For each setting, we design MBP policies that achieve an optimality gap $O\left(\frac{K}{T}+\frac{1}{K}\right)$ per demand unit.
	}
	\label{tab:application_model}
\end{table}


For the ride-hailing application, our assumption that cars relocate immediately is a common simplification in the existing literature \cite[][]{banerjee2016pricing,balseiro2019dynamic}. Moreover, our realistic simulations based on NYC yellow cab data show that our theoretical findings strikingly retain their power even with relocation times, achieving excellent performance over both short and long time horizons (Section \ref{sec:sims}). 

==> commands.tex <==
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
% Editing Notations
%\newcommand{\yk}[1]{}
\newcommand{\yk}[1]{{\color{blue}[YK: #1]}}
\newcommand{\yka}[1]{}%addressed comments
\newcommand{\pq}[1]{{\color{purple}{#1}}} %added paragraph
\newcommand{\pqr}[1]{{\small \color{red}[PQ: #1]}} %response to comments
\newcommand{\pqa}[1]{}%addressed comments
\newcommand{\edit}[1]{{\color{teal} #1}}
\newcommand{\append}[1]{{ #1}} %sentences that says '...is proved in the appendix', for MSOM submission
%\newcommand{\append}[1]{}
\newcommand{\prob}{{\mathbb{P}}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\Ex}{{\mathbb{E}}}

\newcommand{\N}{K} %Number of vehicles
\newcommand{\Iem}{I_{\textup{\tiny em}}}
\makeatletter
\newcommand\footnoteref[1]{\protected@xdef\@thefnmark{\ref{#1}}\@footnotemark}
\makeatother




% Bold Letters
\newcommand{\ba}{\mathbf{a}} %boldface
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\boe}{\mathbf{e}}
\newcommand{\bof}{\mathbf{f}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bz}{\mathbf{z}}


% Bold Face Greek Letters
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\blambdae}{\boldsymbol{\lambda}^{(\epsilon)}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bmue}{\boldsymbol{\mu}^{(\epsilon)}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\hbphi}{\hat{\boldsymbol{\phi}}}

% Calligraphic
\newcommand{\cA}{{\mathcal{A}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cD}{{\mathcal{D}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cN}{{\mathcal{N}}}
\newcommand{\cV}{{\mathcal{V}}}
% Misc
\newcommand{\nK}{\bar{K}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tbq}{\tilde{\mathbf{q}}}
\newcommand{\bbq}{\bar{\mathbf{q}}}
\newcommand{\nq}{\bar{\mathbf{q}}}
\newcommand{\tq}{\tilde{\mathbf{q}}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\MBP}{{\rm {\tiny MBP}}}
\newcommand{\MBPP}{{\rm {\tiny MBP-P}}}

\newcommand{\gJEA}{g_{\rm {\tiny JEA}}}
\newcommand{\gJPA}{g_{\rm {\tiny JPA}}}

\newcommand{\WJEA}{W_{\rm {\tiny JEA}}}
\newcommand{\WJPA}{W_{\rm {\tiny JPA}}}

\newcommand{\JPA}{{\rm {\tiny MBP-JPA}}}
\newcommand{\xF}{{x}^{\rm {\tiny F}}}
\newcommand{\xS}{{x}^{\rm {\tiny S}}}
\newcommand{\xDAG}{{x}^{\rm {\tiny DAG}}}
\newcommand{\zF}{{z}^{\rm {\tiny F}}}
\newcommand{\zS}{{z}^{\rm {\tiny S}}}
\newcommand{\zDAG}{{z}^{\rm {\tiny DAG}}}
\newcommand{\Wopt}{W^{{\rm {\tiny OPT}}}}
\newcommand{\Woptjea}{W^{{\rm {\tiny OPT-JEA}}}}
\newcommand{\Woptjpa}{W^{{\rm {\tiny OPT-JPA}}}}

\newcommand{\Wspp}{W^{{\rm {\tiny SPP}}}}
\newcommand{\aspp}{{\textup{SPP($\bar{\bphi}$)}}}
\newcommand{\sppt}{{\textup{SPP}^t}}

\newcommand{\bxNOM}{\mathbf{x}^{\rm {\tiny Nom}}}
\newcommand{\bxF}{\mathbf{x}^{\rm {\tiny F}}}
\newcommand{\bxS}{\mathbf{x}^{\rm {\tiny S}}}
\newcommand{\bxDAG}{\mathbf{x}^{\rm {\tiny DAG}}}
\newcommand{\bzF}{\mathbf{z}^{\rm {\tiny F}}}
\newcommand{\bzS}{\mathbf{z}^{\rm {\tiny S}}}
\newcommand{\bzDAG}{\mathbf{z}^{\rm {\tiny DAG}}}
\newcommand{\bvJPA}{\bar{v}^{\pi}_{\rm {\tiny JPA}}}
\newcommand{\deq}{\stackrel{.}{=}}
\newcommand{\dsum}{d_{\Sigma}}

\newcommand{\X}{\mathbf{X}} %Sytem state
\newcommand{\e}{\mathbf{e}} %Unit vector
\newcommand{\V}{L} %Lyapunov function
\newcommand{\Vf}{V_{\tiny \textup{finite}}} %nodes with finite buffer
\newcommand{\Vb}{V_{\tiny \textup{b}}} %nodes with finite buffer
\newcommand{\T}{\top} %transpose

\newcommand{\gf}{g_{\tiny \textup{finite}}} %nodes with finite buffer
\newcommand{\ginf}{g_{\tiny \textup{infinite}}} %nodes with finite buffer

\newcommand{\hb}{h_{\tiny \textup{b}}} %nodes with finite buffer

\newcommand{\Cfi}{C_{\tiny \textup{finite}}} %nodes with finite buffer
\newcommand{\Cinf}{C_{\tiny \textup{infinite}}} %nodes with finite buffer
\newcommand{\Cb}{C_{\tiny b}} %nodes with finite buffer

\newcommand{\Df}{D_{\tiny \textup{finite}}} %nodes with finite buffer
\newcommand{\Dinf}{D_{\tiny \textup{infinite}}} %nodes with finite buffer
\newcommand{\Db}{D_{\tiny b}} %nodes with finite buffer

\newcommand{\dsigma}{\bar{d}_{\Sigma}}
\newcommand{\dgap}{\bar{d}_{g}}
\newcommand{\dmin}{\bar{d}_{\min}}


\newcommand{\opt}{\textup{OPT}}

\newcommand{\hx}{\hat{x}}

\newcommand{\nbr}{\mathcal{N}}

\newcommand{\bzero}{\mathbf{0}}

\newcommand{\tbeta}{\tilde{\beta}}
\newcommand{\tphi}{\tilde{\phi}}
\newcommand{\btphi}{\tilde{\boldsymbol{\phi}}}

\newcommand{\ind}{{\mathbb{I}}}
\newcommand{\KL}{\textup{KL}}


\newcommand{\fA}{\bar{\mathbf{A}}} %fluid limit A
\newcommand{\fX}{\bar{\mathbf{X}}} %fluid limit X
\newcommand{\fKX}{\bar{\mathbf{X}}^{\N}} %fluid limit X
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\nbropt}{{\nbr_{{\rm {\tiny opt}}}}}
\newcommand{\conv}{\textup{conv}}
\newcommand*{\fnref}[1]{\textsuperscript{\ref{#1}}}

\newcommand\bnorm[1]{\left\lVert#1\right\rVert}

\makeatletter
\newsavebox\myboxA
\newsavebox\myboxB
\newlength\mylenA

\newcommand*\xoverline[2][0.82]{%
	\sbox{\myboxA}{$\m@th#2$}%
	\setbox\myboxB\null% Phantom box
	\ht\myboxB=\ht\myboxA%
	\dp\myboxB=\dp\myboxA%
	\wd\myboxB=#1\wd\myboxA% Scale phantom
	\sbox\myboxB{$\m@th\overline{\copy\myboxB}$}%  Overlined phantom
	\setlength\mylenA{\the\wd\myboxA}%   calc width diff
	\addtolength\mylenA{-\the\wd\myboxB}%
	\ifdim\wd\myboxB<\wd\myboxA%
	\rlap{\hskip 0.5\mylenA\usebox\myboxB}{\usebox\myboxA}%
	\else
	\hskip -0.5\mylenA\rlap{\usebox\myboxA}{\hskip 0.5\mylenA\usebox\myboxB}%
	\fi}
\makeatother

\newcommand{\mybar}[1]{{\xoverline{.9}{#1}}}




==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
	if (!($root_filename eq $_[0]))
	{
		system( "latexmk -cd -pdf \"$_[0]\"" );
	}
}

==> omlmathbf.tex <==
% OML encoded font for mathrm
% ****************************************************************
%
% :Copyright: Â© 2008, 2010 GÃ¼nter Milde
% :Licence:   This work may be distributed and/or modified under the
%             conditions of the `LaTeX Project Public License`_, either
%             versionÂ 1.3 of this license or (at your option) any later version.
%
% :Identification:
%  ::

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{omlmathbf}
[2011/02/16 v0.1 OML encoded mathbf alphabet]

% Using OML encoded fonts for math alphabets is one way to get
% small Greek letters in different math alphabets (cf. isomath_).

% Requirements
% ------------
%
% Define \alpha .. \Omega as symbols of category ``\mathalpha``::

\RequirePackage{fixmath}

% Options are defined with the key=value interface provided by
% kvoptions_::

\RequirePackage{kvoptions}

% fontfamily
% ----------
%
% Font name, default ``mdput`` (mathdesign utopia)::

\DeclareStringOption[mdput]{fontfamily}

\ProcessKeyvalOptions*

% Implementation
% --------------

% As suggested in `The Comprehensive LaTeX Symbol List`_::

\SetMathAlphabet{\mathbf}{normal}{OML}{\omlmathbf@fontfamily}{b}{n}


% References
% ~~~~~~~~~~
%
% .. _LaTeX Project Public License: http://www.latex-project.org/lppl.txt
% .. _kvoptions: http://mirror.ctan.org/help/Catalogue/entries/kvoptions.html
% .. _isomath: http://mirror.ctan.org/help/Catalogue/entries/isomath.html

